Visual Spatial Description: Controlled Spatial-Oriented Image-to-Text Generation

Image-to-text tasks, such as open-ended image captioning and controllable image description, have received extensive attention for decades. Here, we further advance this line of work by presenting Visual Spatial Description (VSD), a new perspective for image-to-text toward spatial semantics. Given an image and two objects inside it, VSD aims to produce one description focusing on the spatial perspective between the two objects. Accordingly, we manually annotate a dataset to facilitate the investigation of the newly-introduced task and build several benchmark encoder-decoder models by using VL-BART and VL-T5 as backbones. In addition, we investigate pipeline and joint end-to-end architectures for incorporating visual spatial relationship classification (VSRC) information into our model. Finally, we conduct experiments on our benchmark dataset to evaluate all our models. Results show that our models are impressive, providing accurate and human-like spatial-oriented text descriptions. Meanwhile, VSRC has great potential for VSD, and the joint end-to-end architecture is the better choice for their integration. We make the dataset and codes public for research purposes.

==> resources/mapping_table.tex <==
\setlength\tabcolsep{2.5pt}
\begin{table*}[t]
\scriptsize
\begin{center}
\begin{tabular}{llllllllll}
\hline
SpatialSense & above & behind & in & in front of & next to & on & to the left of & to the right of & under\\
\hline
VG & above, above & behind, are & in, are in, are & in front of, are & next to, are & on, are on, are & are left of, in & are to right of & under, are un-\\

& a, above an, & behind, are & in a, are in an, & in front of, are & next to, are & on a, are on & left, in left & on right, on & der, are under\\

& above the, & behind a, be- & are in the, fly- & in front of a, & next to a, are & an, are on the, & side of, left & right of, on & a, are under\\

& are above, are & hind a, behind & ing in, hang- & in front of a, & next to the, & growing on, & of, left side & right side, on & an, below, be-\\

& above a, is & an, behind & ing in, in a, & in front of an, & beside, is next & hanging on, is & of, on left, & right side of, & neath, is un-\\

& above, on top & the, is behind, & in an, in the, & in front of the, & to, is next to & on, is on a, is & on left of, on & right of, right & der, is under\\

& of, over & is behind the, & inside, inside & is in front of & the, next to & on the, laying & left side of, to & side of, to & the, under a,\\

&  & on back of & of, is in, is in &  & a, next to an, & on, lying on, & left, to left of, & right, to right & under an, un-\\

&  &  & a, is in the, &  & next to the, & on a, on a a, & to left of a & of, to right of & der the, un-\\

&  &  & laying in, sit- &  & standing next & on an, on are, &  & a & derneath\\

&  &  & ting in, walk- &  & to & on front of, on &  &  & \\

&  &  & ing in &  &  & the, painted &  &  & \\

&  &  &  &  &  & on, parked &  &  & \\

&  &  &  &  &  & on, printed &  &  & \\

&  &  &  &  &  & on, sitting on, &  &  & \\

&  &  &  &  &  & sitting on top &  &  & \\

&  &  &  &  &  & of, standing &  &  & \\

&  &  &  &  &  & on, walking &  &  & \\

&  &  &  &  &  & on, written on &  &  & \\
\hline
\end{tabular}
\end{center}
\caption{Mapping from predicates of VG-relationship to SpatialSense labels.}
\label{tab:app1}
\end{table*}
